Information Leakage Games

We consider a game-theoretic setting to model the interplay between attacker and defender in the context of information flow, and to reason about their optimal strategies. In contrast with standard game theory, in our games the utility of a mixed strategy is a convex function of the distribution on the defender's pure actions, rather than the expected value of their utilities. Nevertheless, the important properties of game theory, notably the existence of a Nash equilibrium, still hold for our (zero-sum) leakage games, and we provide algorithms to compute the corresponding optimal strategies. As typical in (simultaneous) game theory, the optimal strategy is usually mixed, i.e., probabilistic, for both the attacker and the defender. From the point of view of information flow, this was to be expected in the case of the defender, since it is well known that randomization at the level of the system design may help to reduce information leaks. Regarding the attacker, however, this seems the first work (w.r.t. the literature in information flow) proving formally that in certain cases the optimal attack strategy is necessarily probabilistic.

==> reviews.tex <==
\begin{verbatim}
----------------------- REVIEW 1 ---------------------
PAPER: 70
TITLE: Information Leakage Games
AUTHORS: M\UTF{00E1}rio S. Alvim, Konstantinos Chatzikokolakis, 
Yusuke Kawamoto and Catuscia Palamidessi

Overall evaluation: 3 (strong accept)

----------- Overall evaluation -----------
The paper studies a game-theoretic setting modelling the interplay
between an attacker and a defender in the context of information 
flow. The aim of the work is to study optimal strategies in this 
setting. The setting is different to standard game theory,
in particular here the utility of a mixed strategy is a convex 
function of the distribution of the defender's pure actions, 
rather than the expected value of their utilities. The main 
result of the work is to show the existence of a Nash equilibrium 
in this framework.

overall very strong paper which analyzes an interesting security 
problem and provides an original game theoretical framework for 
solving the problem. The reflection about why independence fails 
for confidentiality, i.e. that composing leaky channels may result 
in a secure channel is a beautiful insight that (negatively) 
relate a basic technical axiom of game theory with a fundamental 
property of confidentiality. This framework seems also of interest 
to the general game theory community.
Strong accept

some comments:

"active attacker": I think "interactive" is the right term.
"passive attacker"= attacker that can only eavesdrop
"active attacker" = attacker that can provide public inputs 
(e.g. plain text messages in crypto communication): most QIF 
works study active attackers "interactive attacker"= attacker 
that interact with the system and this interaction includes 
memory and feedback (only few works e.g. [8,28])
\end{verbatim}

\commentMA{Done.}

\begin{verbatim}
"the pure strategies d, a are not always optimal" what do you 
mean? d=0 is a pure strategy but d in itself is not
\end{verbatim}

\commentMA{Done.}

\begin{verbatim}
what do you mean with "binary sum": is it boolean or? 
exclusive or? please clarify.
\end{verbatim}

\commentMA{Done.}

\begin{verbatim}
(cf 2.3) you seem to refer to theorem 1 which is in sec 2.2.
\end{verbatim}

\commentMA{Done.}

\begin{verbatim}
----------------------- REVIEW 2 ---------------------
PAPER: 70
TITLE: Information Leakage Games
AUTHORS: M\UTF{00E1}rio S. Alvim, Konstantinos Chatzikokolakis, 
Yusuke Kawamoto and Catuscia Palamidessi

Overall evaluation: 2 (accept)

----------- Overall evaluation -----------
This paper considers a game between two players where a defender 
wants to communicate some private message x but does not want 
to leak x to an adversary (i.e., attacker). The defender can 
randomize among multiple actions and so is the attacker. 
The paper models this interaction between the defender and 
attacker as a zero-sum game where the utility is a measure of 
information leakage, termed Bayesian vulnerability. 
\end{verbatim}

\commentMA{Done.
\ \\
\ \\
(We capture more than Bayes vulnerability,
but we decided to ignore this comment)}

\begin{verbatim}
The authors show that players’ utility is convex in the 
defender’s mixed strategy and linear in the attacker’s mixed 
strategy. Therefore, standard minimax approach can be applied 
to solve the game. Finally, the paper takes a case study on a 
MANET instance with 30 users and exhibits the minimax strategy 
computed by their algorithm.

Overall, I found the idea of modeling the information leakage 
as player’s utility of a game interesting. Given this modeling, 
the proof of equilibrium existence and computational techniques 
in the paper are not surprising due to Von Neumann’s minimax 
theorem.

One concern I had is that the assumption that the information 
leakage measure has to be convex seems not very well justified, 
though the authors said that this has been used before in other 
work. 
\end{verbatim}

\commentMA{
Done.
\ \\
\ \\
(We decided to leave the text as it is.
Right now we have a brief explanation of why 
vulnerabilities must be convex in Footnote~\ref{footnote:convex}.
Should we make it more clear in the main text?
This is probably something people from Security don't know 
about, but I suspect people from Game Theory are more likely
to know about.)}

\begin{verbatim}
For example, in the two-billionaires example, why the 
maximum of each column is a good quantity to consider?
The authors may want to give more explanation about this part 
since this modeling part is a major contribution of this paper 
(at least seems to me).
\end{verbatim}

\commentMA{Done.}

\begin{verbatim} 
Another question I had is that what if the space for defender 
and attacker actions are exponentially large so that directly 
solving the game via minimax becomes computationally prohibited. 
This seems natural in applications. For example in the MANET 
example, the defender only sends a message to one of his 
neighbors, but what if the defender can choose k neighbors 
to send his message? I think this makes the problem 
computationally more interesting.
\end{verbatim}

\commentMA{Done.}

\begin{verbatim} 
Some detailed information in the case study is missing. 
For example, how did you compute the C(x,y) since the users are 
moving in the network and there is a stochastic process during 
the procedure by randomly influencing neighbor nodes. How 
realistic is Crowds protocol? Are there any other protocols? 
\end{verbatim}

\commentMA{Done.}

\begin{verbatim} 
The Utility in Table 9 seems to not vary much in each column. 
Instead of a case study in a small instance, the paper may want 
to justify their model in a more realistic real-world instance.
\end{verbatim}

\commentMA{Done.}

\begin{verbatim}
Other comments:
This paper should point out at the beginning that the game 
considered in this paper is a zero-sum game. 
The current description is a bit confusing since words like 
"Nash equilibrium", "equilibrium existence" naturally make 
readers think that this is a general-sum game. 
\end{verbatim}

\commentMA{Done.}

\begin{verbatim} 
Moreover, I found the term "optimal defender strategy" also a bit 
confusing until I realized that the game is zero-sum.
\end{verbatim}

\commentMA{Done.}

\begin{verbatim} 
In the contribution parts, "Nevertheless, we show that the 
fundamental results of game theory, notably the minimax theorem 
and the existence of Nash equilibria, still hold for
our games.": given the convex-affine utility structure, this 
follows from previous work, not a very new contribution.
\end{verbatim}

\commentMA{Done.}

\begin{verbatim} 
Section 4.2, third line: which is also based convex ... based on?
\end{verbatim}

%\commentMA{To do.}
\replyYK{Already fixed}

\begin{verbatim} 
Rightly above Section 7: "However, in our experiments we found 
that this conversion leads
to a substantially large problem," what is the problem by 
linearizing the piecewise linear function?
\end{verbatim}

\commentMA{Done.}

\begin{verbatim} 
Reference 67 is not correct.
\end{verbatim}

%\commentMA{To do.}
\replyYK{This was [47], which is fixed and now [19].}

